Learning Dynamic Bipedal Walking Across Stepping Stones

In this work, we propose a learning approach for 3D dynamic bipedal walking when footsteps are constrained to stepping stones. While recent work has shown progress on this problem, real-world demonstrations have been limited to relatively simple open-loop, perception-free scenarios. Our main contribution is a more advanced learning approach that enables real-world demonstrations, using the Cassie robot, of closed-loop dynamic walking over moderately difficult stepping-stone patterns. Our approach first uses reinforcement learning (RL) in simulation to train a controller that maps footstep commands onto joint actions without any reference motion information. We then learn a model of that controller's capabilities, which enables prediction of feasible footsteps given the robot's current dynamic state. The resulting controller and model are then integrated with a real-time overhead camera system for detecting stepping stone locations. For evaluation, we develop a benchmark set of stepping stone patterns, which are used to test performance in both simulation and the real world. Overall, we demonstrate that sim-to-real learning is extremely promising for enabling dynamic locomotion over stepping stones. We also identify challenges remaining that motivate important future research directions.

==> related_work.tex <==
% !TEX root =  paper.tex
\section{Related Work} 
Dynamic bipedal walking over discrete terrains require the controllers to deliberately targeting each footstep, traveling at decent speed, while maintaining balance. Several previous works focus on using model-based techniques to design controllers, such as using an offline gait library and online interpolation \cite{Nguyen2017a, Nguyen2020}, control barrier function \cite{Nguyen}, or using reduced-order models \cite{Dai2021}. These techniques often involve a sequence of optimizations that have to be computed online. Toward similar goals, recent learning-based techniques show that RL can produce learned control policies that enable legged robots to walk over discrete terrains using curriculum-based training \cite{Xie2020a} or hierarchical control structure \cite{Xie2021, Yu2021, Margolis2021, Tsounis2019, Gangapurwala2020}. It is still unclear how these learning techniques can carry out to the real-world demonstrations of bipedal robot dynamically walking over stepping stones. 

% \textbf{Dynamic Bipedal Locomotion on Footstep-constrained Environments.} \\
% Using offline trajectories and online interpolation \cite{Nguyen2017a, Nguyen, Nguyen2020}
% Using simplified models to plan \cite{Dai2021}

% \textbf{RL for Legged Locomotion with Terrain Constraints.}\\ 
% Bipedal simulation stepping stones \cite{Xie2020a, Peng2017}
% Quad sim \cite{Tsounis2019, Gangapurwala2020}
% Quad sim2real Using existing controller as hierarchical structure \cite{Xie2021, Yu2021, Margolis2021}.

% \textbf{Learning Representation Model for Bipedal Locomotion.} 
% Simple model with 2D terrain \cite{Sanghvi}. quad \cite{Li2021a}
